CaVE: A Constraint Storage Approach to Handling Integrity Constraints

This paper presents Constraints as Verifiers and Emitters (CaVE), a constraint storage approach for handling integrity constraints in stableKanren. stableKanren is a normal logic-program solver based on extended unification and resolution. Integrity constraints control the outcomes of goals in normal logic programs, which is critical for non-monotonic reasoning. There is no resolution-based algorithm for handling integrity constraints that can be used in stableKanren. Therefore, we design Constraints as Verifiers and Emitters (CaVE), a constraint storage that works with resolution to support integrity constraints. We discuss variants of CaVE with respect to the integrity constraints, ranging from propositional to grounded and predicate versions. We implement CaVE using Scheme in stableKanren and show a series of example normal programs written in stableKanren with integrity constraints.

==> eptcsdata.tex <==
\providecommand{\firstpage}{444}
\providecommand{\publicationstatus}{W. Faber, L. Giordano, R. Rocha, V. Santos Costa (Eds.):\\ 42nd International Conference on Logic Programming (ICLP 2026)\\
EPTCS 450, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.450.32}{10.4204/EPTCS.450.32}}
\pdfoutput=1

